Facial Depth and Normal Estimation using Single Dual-Pixel Camera

Many mobile manufacturers recently have adopted Dual-Pixel (DP) sensors in their flagship models for faster auto-focus and aesthetic image captures. Despite their advantages, research on their usage for 3D facial understanding has been limited due to the lack of datasets and algorithmic designs that exploit parallax in DP images. This is because the baseline of sub-aperture images is extremely narrow and parallax exists in the defocus blur region. In this paper, we introduce a DP-oriented Depth/Normal network that reconstructs the 3D facial geometry. For this purpose, we collect a DP facial data with more than 135K images for 101 persons captured with our multi-camera structured light systems. It contains the corresponding ground-truth 3D models including depth map and surface normal in metric scale. Our dataset allows the proposed matching network to be generalized for 3D facial depth/normal estimation. The proposed network consists of two novel modules: Adaptive Sampling Module and Adaptive Normal Module, which are specialized in handling the defocus blur in DP images. Finally, the proposed method achieves state-of-the-art performances over recent DP-based depth/normal estimation methods. We also demonstrate the applicability of the estimated depth/normal to face spoofing and relighting.

==> Rebuttal/rebuttal_fig1.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]{Rebuttal/AdditionalResults.pdf}
\vspace{-3mm}
\caption{
% \textbf{Additional results.} 
(a) Refined face relighting by smoothing normal (\rone). (b) Feature refinement by ASM (\rtwo).
% \jaesung{@MJ: replace bottom right figs? or mask our the bg normals.}
}
\label{fig:additional_rebuttal}
\vspace{-4mm}
\end{figure}

==> Rebuttal/rebuttal_fig2.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]{Rebuttal/DepthandNormal.pdf}
\vspace{-3mm}
\caption{
{Depth and normal results in the wild (\rthree).} (a) public DP dataset [\textcolor{red}{2}], and (b) our captured natural DP images. 
}
\label{fig:additional_rebuttal2}
\vspace{-4mm}
\end{figure}

==> Rebuttal/rebuttal_table1.tex <==
\vspace{-4mm}
\begin{table}[!h]
\centering
\scriptsize
\caption{{Symbols' dimensions.} P$({=}4)$, M$({=}16)$, and C$({=}32)$.}
\vspace{-6mm}
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{cccccc}
\\ \Xhline{1.5\arrayrulewidth}
Symb & $\mathcal{F}$,$\mathcal{G}$ & $\mathcal{V}$,$\mathcal{V}_\mathcal{S}$, $\mathcal{W}$  & $\mathcal{C}_\mathcal{A}$ & $\mathcal{C}_\mathcal{S}$ & $\mathcal{C}_\mathcal{N}$ 
\\ \hline
dim    & (C,H,W) & (C,3,H,W) & (C,M,H,W) & (C,P,H,W) & (M,2C,H,W)
\\ \Xhline{1.5\arrayrulewidth}
\end{tabular}
%\vspace{-3.5mm}
% \caption{\textbf{symbols' Dimension.} P$(=4)$ is the number of sampled points, M$(=12)$ is disparity range, C$(=32)$ is channel length.} 
\label{tab:dimension}
\vspace{-4mm}
\end{table}

==> Rebuttal/rebuttal_table2_normal.tex <==
% \vspace{-2mm}
\begin{table}[!t]
\centering
\scriptsize
\caption{{Ablation study for normal estimation schemes (\rthree).}}
\vspace{-4mm}
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{rl|cc}

\Xhline{4\arrayrulewidth}

\multicolumn{2}{c|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{normal performance (lower the better)} 
\\

& & ~~~~MAE~~~~ & RMSE 
\\ \Xhline{2\arrayrulewidth}

\rowcolor{yellow!20} Surface normal from & ANM (ours) & ~~7.479~~~~~~~~~~~~~~~~ & 9.386~~~~~~~~~~~~~~ 
\\ % \Xhline{1\arrayrulewidth}

% & NNet~[34] & ~~9.634~(\textcolor{purple}{$\uparrow$ 2.155}) & 11.877~(\textcolor{purple}{$\uparrow$ 2.491})
% \\

% & depth of ASM & ??~(\textcolor{purple}{$\uparrow$ ??.?}) & ??.?~(\textcolor{purple}{$\uparrow$ ??.?}) \\

& depth of ASM ($\hat{d}$) & 10.828~(\textcolor{purple}{$\uparrow$ 3.349}) & 12.472~(\textcolor{purple}{$\uparrow$ 3.086}) \\

\Xhline{4\arrayrulewidth}

\end{tabular}
\label{tab:normal-from-depth}
\vspace{-6mm}
\end{table}

==> __header.tex <==
% Beautiful table
% \usepackage{times}
\usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{verbatim}
\usepackage{hhline}
% \usepackage{makecell}
% \usepackage{paralist}
% \usepackage{booktabs}
\usepackage{adjustbox}
\usepackage{float}
\usepackage{cite}

%%% Tables (jaesungchoe 2022.March.04)
\usepackage{hhline}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{graphicx}

%%% \st{..}
\usepackage{ulem}

\usepackage{algorithm}
\usepackage{algorithmic}
% \usepackage[utf8]{inputenc}
% \usepackage{geometry}
\usepackage{algpseudocode}

% cell color
% usepackage[table]{xcolor}% http://ctan.org/pkg/xcolor
\usepackage{xcolor,colortbl}
\newcommand{\first}[1]{\cellcolor{yellow!75}\textbf{#1}}
\newcommand{\second}[1]{\cellcolor{yellow!25}{#1}}

\definecolor{gray}{rgb}{0.5, 0.5, 0.5}
\definecolor{darkgray}{rgb}{0.2, 0.2, 0.2}
\definecolor{scarlet}{rgb}{1, 0.35, 0.15}
\definecolor{mulberry}{rgb}{0.773, 0.294, 0.549}
\definecolor{blue}{rgb}{0, 0, 1}
\definecolor{skyblue}{rgb}{0.3, 0.7, 0.9}
\definecolor{darkgreen}{rgb}{0.2, 0.7, 0.1}
\definecolor{darkyellow}{rgb}{1, 0.65, 0}

% Optional math commands from https://github.com/goodfeli/dlbook_notation.
% \input{math_commands.tex}

% \usepackage{hyperref}
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref} % letterpaper=true,
% \usepackage{url}

\usepackage{xspace}

% middle lines.
\usepackage{soul}

% \cmark
% https://tex.stackexchange.com/questions/42619/x-mark-to-match-checkmark/42620
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{{vs}\onedot}
\def\wrt{\emph{w.r.t}\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\def\aka{\emph{a.k.a}\onedot}


% https://www.overleaf.com/project/5c3ee6aa83e7382dd5ccc228
\newcommand{\Tref}[1]{Table~\textcolor{blue}{\ref{#1}}}
\newcommand{\Eref}[1]{Eq.~\textcolor{blue}{\ref{#1}}}
\newcommand{\Fref}[1]{Fig.~\textcolor{blue}{\ref{#1}}}
\newcommand{\Sref}[1]{Sec.~\textcolor{blue}{\ref{#1}}}
\newcommand{\Aref}[1]{Alg.~\textcolor{blue}{\ref{#1}}}

%% Define new markers
\newcommand{\cvpr}[1]{\textcolor{purple}{cvpr $>$ #1}}
\newcommand{\JS}[1]{\textcolor{magenta}{jaesung $>$ #1}}
\newcommand{\MJ}[1]{\textcolor{blue}{MJ $>$ #1}}


% Footnote without marker
% https://tex.stackexchange.com/questions/30720/footnote-without-a-marker
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

% \usepackage[pagebackref]{hyperref}
% colorlinks 
% breaklinks


% Support for easy cross-referencing
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}


==> figure/fig_arch/anm_arch.tex <==
\begin{figure}
\centering
\includegraphics[width=0.97\linewidth]{figure/fig_arch/ANMFigure_cropped.pdf}
\vspace{-2mm}
\caption{\textbf{Architecture of ANM.} Adaptive Normal Module consists of a surface sampling and a 3D deformable convolutional layer for surface normal regression.}
\label{fig:ANM}
\vspace{-5mm}
\end{figure}

==> figure/fig_arch/asm_arch.tex <==
\begin{figure}
\centering
\includegraphics[width=0.97\linewidth]{figure/fig_arch/ASMFigure_cropped.pdf}
\vspace{-2mm}
\caption{\textbf{Architecture of ASM.} Adaptive Sampling Module consists of a dynamic sampling and a self-3D attention layer.}
\label{fig:ASM}
\vspace{-5mm}
\end{figure}

==> figure/fig_outdoors/applications.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.99\linewidth]{figure/fig_outdoors/Applications3_cropped.pdf}
\vspace{-2mm}
\caption{\textbf{Applications.}
(a) To show the application to face anti-spoofing, StereoDPNet infers depth maps with the real and fake face samples (paper attack and display attack). Note that the depth maps from StereoDPNet allow the face detector to distinguish whether the input is a real face or not because it computes correspondences between two DP images.
(b) We display the original DP image, estimated normal map from StereoDPNet, and two different relit images with sampled lighting directions.
}
\label{fig:applications}
\vspace{-4mm}
\end{figure*}

==> table/facespoofing.tex <==
\begin{table}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{10pt}
\begin{tabular}{ccccc}
\\ \Xhline{3\arrayrulewidth}
Method & Acc $\uparrow$ & ACER $\downarrow$ & FP & FN 
\\ \Xhline{1\arrayrulewidth}
PRNet~\cite{feng2018prn} & 62.815 & 0.5083 & 38 & 97
\\ \hline
\textbf{Ours} & \textbf{100.0} & \textbf{0.0000} & \textbf{0} & \textbf{0} \\ \Xhline{3\arrayrulewidth}
\end{tabular}
\caption{\textbf{Face spoof detection results} Evaluation results from a pretrained FeatherNet using depth from PRNet (Monocular) and Ours (DP data) on 608 true and 266 fake samples. ACER is the error rate of classifying face widely used in~\cite{zhang2019feathernets, wang2020deep}. FP and FN denote False Positive and False Negative sample numbers.}
\label{tab:facespoofingtable}
\vspace{-8mm}
\end{table}
